Data Makes Better Data Scientists

With the goal of identifying common practices in data science projects, this paper proposes a framework for logging and understanding incremental code executions in Jupyter notebooks. This framework aims to allow reasoning about how insights are generated in data science and extract key observations into best data science practices in the wild. In this paper, we show an early prototype of this framework and ran an experiment to log a machine learning project for 25 undergraduate students.

==> analysis.tex <==
\section{Preliminary Analysis} \label{sec:analysis}

\begin{table}
    \centering
    \footnotesize
    \begin{tabularx}{0.7\columnwidth}{ll}
    \hline
          & Percentage of Logs (\%)  \\
          \hline
         Hidden Cells &  37.16 \\
         Final Notebook Cells &  62.84 \\
    
    \end{tabularx}
    \caption{The distribution of cell runs that was not present in the final notebook}
    \label{tab:hidden}
\end{table}

\begin{table}
    \centering
    \footnotesize
    \begin{tabularx}{0.7\columnwidth}{ll}
    \hline
          & Percentage of Logs (\%)  \\
          \hline
         No Error & 82.93 \\
         Format Error & 1.01 \\
         Execution Error & 16.06 \\
        
    \end{tabularx}
    \caption{The distribution of Python errors in cell runs over all students}
    \label{tab:errors}
\end{table}


We performed a preliminary analysis to characterize the workflows from information gathered in the student logs. This section summarizes some key insights gained from our system.

\vspace{0.5em} \noindent \textbf{$37\%$ of cell runs are not represented in the final notebook.} It can be observed in Table \ref{tab:hidden} that approximately $37\%$ of cell runs captured in the log are not represented in the final submitted notebook across all students. This suggests that a significant part of the written code is ``lost'' upon final submission. We hope that tracking and characterizing this code in our system will allow a greater understanding of processes in data science.

\vspace{0.5em} \noindent \textbf{$16\%$ of cell executions results in Python execution errors.} Table \ref{tab:errors} shows the distribution of Python errors across all logs. While format errors only represent $1\%$ of the total cells ran, execution errors make up $16\%$ of the distribution. To the best of our knowledge, no prior work has studied the impact of errors on the overall data science workflow. We are particularly interested in how a user addresses error statements and whether these error statements lead to changes in the code that generates new insights.

\vspace{0.5em} \noindent \textbf{Behavior significantly varies between student workflows.} In Figure \ref{fig:time}, we can observe the timeline of when each student executed cell runs relative to their first execution. The students generally worked on the project across multiple days, with significant breaks between sessions. There is a high variance between the time spent by each student. Our system would allow us to characterize and correlate that variance with final outcomes. We also hypothesize that there may be user pivots in the project between breaks that can be characterized by the code log. These temporal breaks may be a strong signal for how to break up a complete project into mini-processes, as described in Section~\ref{sec:arch}. 




\vspace{0.5em} \noindent \textbf{Some column attributes are significantly more referenced than others.} We matched exact references made in each code cell in the logs to column attributes. The distribution of these matches is shown in Figure \ref{fig:columns}, describing the percentage of cell runs that contained references to each attribute. ``DepDel15'' is referenced particularly frequently ($31\%$ of all cell runs), which is expected since that is the target variable. More surprisingly, ``DayOfWeek'', ``Distance'' and ``Origin'' are all referenced in >4\% more cells than other attributes. This insight from our system allows us to directly reason about the importance of different data columns from user behavior.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\columnwidth]{figures/timeline.png}
    \caption{The timeline of when students ran the cells relative to when they executed the first cell}
    \label{fig:time}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{figures/column_references.png}
    \caption{The distribution of column attribute references overall cell runs}
    \label{fig:columns}
\end{figure}


% \jz{I omitted the f1-score graph because that was the least interesting to discuss. Additionally, I didn't color-code the time graph with f1-score, because I think that wasn't a correlation we should strongly state.}
% We show a histogram of F1-scores on the testing dataset in Figure \ref{fig:accuracy} for 20 students. For five students, there were errors in the final testing file that was submitted, and we were not able to extract the F1-score. We observed some of these students submitted the predictions on the training datasets or falsely sampled the testing dataset. Of the students with valid submissions, there is a significant variance in the F1 score. This gives us a final metric to measure the   ``success'' of the task between students for this experiment. 


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.8\columnwidth]{figures/f1_score.png}
%     \caption{Histogram of final F1-score for 20 students (5 students were not included since they did not submit the correct testing file)}
%     \label{fig:accuracy}
% \end{figure}

==> challenges.tex <==
\section{Limitations and Challenges}\label{sec:challenges}
With the goal of identifying common practices in data science projects, we proposes a framework for logging and understanding incremental code executions in Jupyter notebooks.  Our initial experiment focused on a standard  machine learning task with novice data scientists. This setting was practical since it had clear final performance metrics (accuracy on the testing dataset) and a captive audience (undergraduate students). However, this is not the only possible data science setting and may not represent industrial use-cases. The pilot study is meant to illustrate the scope of data and insights that are possible with our logging and analysis framework.

 \vspace{0.5em} \noindent \textbf{Direction 1. More Complex Tasks. } We would like to ask the community for direction on potential future experiments to expand the setting of our insight. We are currently considering three possible directions: (1) the same machine learning task with data science experts to compare workflow differences between students and experts, (2) increasing the complexity of data discovery/integration needed to perform the task, and/or (3) increasing the complexity of machine learning needed to perform the task. Feedback on which of these potential experiments are most valuable to the community is welcome.

 \vspace{0.5em} \noindent \textbf{Direction 2. Logging Scope} Section \ref{sec:setup} describes the design decisions that went into what information was recorded in our execution log. This information was shaped by what was easily captured and what was necessary to answer our proposed initial questions about data science workflows. We can highlight two significant sources of information that are not tracked: (1) notebook outputs and (2) tools outside of Jupyter notebooks. Specifically, in the second case, there are many places where a data scientist can gain insights for their task outside the Jupyter notebook environment. Tools like Excel~\cite{msexcel} allows visualizations of the data. Online resources such as Kaggle or Stack Overflow~\cite{kaggle, stack_overflow} provide previous sample code. Novel large language machine learning models~\cite{codex, gpt} can now generate task-specific code that pieces together insights from disparate origins. These tools can shape the workflow of the data science process in ways not captured by the execution log. We invite the HILDA community to discuss the significance of all these sources of information and capture techniques for recording influences outside of the Jupyter environment.

 \vspace{0.5em} \noindent \textbf{Direction 3. Towards Data Science KPIs. } Our preliminary analysis in Section \ref{sec:analysis} focuses on characterizing the data gathered in the initial experiment. We are in the process of performing further analysis to link this data to general questions about data science and create metrics (KPIs) for assessing data scientists as they perform their tasks. There are currently some important questions that we would like to tackle:
\begin{itemize}
    \item What is the actual time spent on different parts of the data science process (e.g., cleaning, visualization, model-tuning)?
    \item What are simple common blockers/errors from amateur data scientists?
    \item How important is visualization in data science? What types of visualizations are used, and is there a difference between the different types?
    \item Which features made it to the final model? How much time is spent on features not in the final model?
    \item Can we capture pivots in the data science workflow and reason about what caused those pivots?
\end{itemize}

We would like insight from the community on interest in these questions and any additional significant questions on data science workflows. 
